Stein Variational Goal Generation for adaptive Exploration in Multi-Goal Reinforcement Learning

In multi-goal Reinforcement Learning, an agent can share experience between related training tasks, resulting in better generalization for new tasks at test time. However, when the goal space has discontinuities and the reward is sparse, a majority of goals are difficult to reach. In this context, a curriculum over goals helps agents learn by adapting training tasks to their current capabilities. In this work we propose Stein Variational Goal Generation (SVGG), which samples goals of intermediate difficulty for the agent, by leveraging a learned predictive model of its goal reaching capabilities. The distribution of goals is modeled with particles that are attracted in areas of appropriate difficulty using Stein Variational Gradient Descent. We show that SVGG outperforms state-of-the-art multi-goal Reinforcement Learning methods in terms of success coverage in hard exploration problems, and demonstrate that it is endowed with a useful recovery property when the environment changes.

==> intro_olivier.tex <==
\section{Introduction}

In standard Reinforcement Learning (RL), agents learn a policy to optimally achieve a single task. By contrast, in Multi-goal RL \citep{kaelbling1993learning}, they address a set of tasks by having policies conditioned on goals, where each goal corresponds to an individual task. The resulting goal-conditioned policies offer an efficient way for sharing experience between related tasks \citep{schaul2015universal}. While targeting a goal, an agent may achieve another goal. Besides, the agents do not know in advance whether the goal it is targeting is {\em valid}, i.e. whether it can be achieved or not. Finally, the general ambition in the multi-goal RL context is to obtain an agent able to reach any goal from some desired goal distribution and to do so reliably and efficiently. This is particularly challenging in settings where the desired goal distribution is unknown at train time, which means discovering the space of valid goals by experience and optimizing its coverage without any prior knowledge. 

To avoid deceptive gradient issues and a tedious reward engineering process, multi-goal RL often considers the sparse reward context, where the agent only obtains a non-null learning signal when the goal is achieved. In that case, the multi-goal framework makes it possible to leverage Hindsight Experience Replay (\her) \citep{andrychowicz2017hindsight} which helps densify the reward signal by relabeling failures as successes for the goals achieved by accident.
However, in settings with discontinuities in the goal space (e.g., walls in a maze), or in hard exploration problems where the long task horizon results in an exponential decrease of the learning signal \citep{osband2016generalization}, many goals remain hard to achieve and using \her does not suffice to reach all valid goals.

In these more difficult contexts, and without any desired goal distribution at hand, we want to maximize a metric that we call {\em success coverage}\footnote{The same metric is called {\em competence} in \cite{blaes2019control} and {\em feasibility} in \cite{racaniere2019automated}.} which measures the performance of the agent on all valid goals. This metric encompasses the capacity of the agent to explore and master every valid goal in the environment.
To do so, the selection of goals must be structured into a curriculum to help agents explore and learn progressively by adapting training tasks to their current capabilities \citep{colas2022autotelic}. The question is: how can we organize a curriculum of goals to maximize the success coverage?

A first approach consists in focusing on novelty, with the objective of expanding the set of achieved goals. This is the approach of \rig \cite{nair2018visual}, \discern \cite{warde2018unsupervised}, \skewfit\cite{pong2019skew} and \mega as well as \omeg \cite{pitis2020maximum}. This leads to strong exploration results, but success coverage is only optimized implicitly.

Another strategy is to bias the goal generation process toward goals of intermediate difficulty (GOIDs). The general intuition is that addressing goals that are too easy or too hard does not foster progress, thus the agent needs to identify goals on which it can make some progress. The focus is thus more on performance. This is the approach of asymetric self-play \cite{sukhbaatar2017intrinsic}, \ggan \cite{florensa2018automatic}, \setso \cite{racaniere2019automated} or \vds \cite{zhang2020}. By aiming at performance, those methods target more explicitly success in encountered goals, but benefit from implicit exploration.


In this work, we propose a novel method which provides the best of both worlds. Our method, called \svgg\footnote{For Stein Variational Goal Generation. Code and instructions to reproduce our results will be made publicly available at \href{https://anonymous.4open.science/r/Stein-Variational-Goal-Generation-1A6E}{https://anonymous.4open.science/r/Stein-Variational-Goal-Generation-1A6E}.}, learns a model of the probability of succeeding in achieving goals by relying on a set of particles where each particle represents a goal candidate. This set of particles is updated via Stein Variational Gradient Descent \citep{svgd} to fit GOIDs, modeled as goals whose success is the most unpredictable. A key feature of \svgd is that the gradient applied to particles combines an attraction term and a repulsion term which help strike a good balance between exploration and exploitation. In particular, when the agent cannot find any additional GOID, due to the repulsion term of \svgd, the current particles repel one another resulting in fostering more exploratory goal sampling.
This endows \svgg with a very flexible model of the current capabilities of the corresponding  agent. Based on this feature, we formally demonstrate that \svgg possesses a very useful \textit{recovery property} that prevents catastrophic forgetting and enables the agent to adapt when the environment changes during training. We empirically validate \svgg on Multi-goal RL problems where the goal spaces is of moderate size, and leave investigations on problems where goals are images for future work.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rl_olivier.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}

In this section we investigate the relationships between our \svgg algorithm and two strongly related algorithms, \mega and \ggan, that we use as baselines.

\subsection{Relationship to MEGA}

Similarly to \discern \citep{warde2018unsupervised} which directly samples behavioral goals from a replay buffer of achieved goals, \mega builds an explicit model of these goals. In more details, \mega \citep{pitis2020maximum} (1) maintains a buffer of previously achieved goals, (2) models the distribution of achieved goals via a kernel density estimation (KDE), and (3) samples behavioral goals from the replay buffer in low density regions of this distribution.

Rather than this model of achieved goals, \svgg builds an explicit model of the capability of the agent to achieve goals, and focuses on the region where goal achievement is the most unpredictable. 

A key difference between \mega and \svgg is that the way \svgd optimization is performed in the latter guarantees that the particles --~or sampled behavioral goals~--, keep flexibly covering the goal space, achieving a good balance between looking for novelty and preventing catastrophic forgetting.

Besides, due to \svgd optimization, behavioral goals sampled by \svgg may have never been achieved before. Thus, \svgg needs a validity prior similar to the validity loss of the \setso algorithm \cite{racaniere2019automated}. 

\subsection{Relationship to GoalGAN}

Instead of using an explicit model of achieved goal, one can obtain an implicit model with a generative approach. For instance, \rig \citep{nair2018visual} and \skewfit \citep{pong2019skew} use variational auto-encoding \citep{kingma2013auto} of the achieved goal distribution.
Rather than using a VAE, one can learn a goal generator using an adversarial method that generates behavioral goals at the frontier of the agent's capabilities. This is the approach taken in \ggan \citep{florensa2018automatic}. In more details, \ggan samples goals from the buffer of achieved goals so as to obtain goals of intermediate difficulty (GOIDs). A discriminator sorts out non GOIDs from GOIDs, and a generator produces goals that fool the discriminator. While appealing, the approach is prone to instabilities, with a generator that may usually diverge far from the space of valid goals.

The \svgg algorithm also samples GOIDs, but it does so by learning a predictive model of the agent's goal achievement capability and building a sampling distribution that focuses on goals whose achievement is the most unpredictable.
Because it does not call upon an adversarial generative process, \svgg is less prone to instabilities.

%\setso \citep{racaniere2019automated} stands as an extension of \ggan, where a goal setter is learned to provide goals of various levels of difficulty w.r.t. a judge network (similar to our success predictor, see next section). The provided goals remain close to already achieved goals, and are diverse enough to avoid mode collapse. This approach suffers from relying on invertible networks to map from the latent space to the goal space, which severely limits the modeling power, and can reveal problematic for high dimensional goal spaces, e.g. images. 

%Asymmetric self-play \citep{sukhbaatar2017intrinsic} is another way to generate goals, with a teacher agent seeking to produce goals that are just beyond the capabilities of the student agent. Both teacher and student learn simultaneously, with an equilibrium of adverse rewards determined on their respective time to go. However, this balance is hard to maintain, and many useful areas are missed. 

%Finally, curiosity-driven exploration \citep{pathak2017curiosity} could be placed in that adversarial category, with an inverse model that aims at learning a compact latent representation space from which it is still possible to predict the dynamics of the environment. The agent is then rewarded for exploring areas whose dynamics are hard to predict. Nevertheless, it requires complex model learning and may lead to hallucinations for the agent which can remain stuck in difficult areas of the search space, by contrast with our simpler model-free setting.   

%variante de OMEGA qui se restreint aux buts interessants pour la desired : \citep{abs-2109-08903}

%\paragraph{Skills Discovery} Many recent works propose to deal with the problem of exploration based on a quantization of the state space in distinct skills, that are supposed to correspond to homogeneous sets of states that can be achieved with similar policies. Based on variational empowerment \citep{gregor2016variational, choi2021variational} that approximates a posterior skill distribution via variational inference and  mutual information maximization, \diayn \citep{eysenbach2018diversity} leverages a discriminator network to identify for each trajectory the skill that the agent is currently using. Extensions such as   \cite{kamienny2021direct} propose to sequentially chain skills to deal with hard environments. However, these approaches are unstable, and the full exploration of the environment is not guaranteed.  

%\paragraph{Population-based Exploration} Population-based RL, using evolutionary strategies to explore environments, is receiving increasing attention for hard exploration problems. Methods such as Novelty Search or Quality Diversity \citep{conti2018improving,liu2018pns,paolo2021sparse} deal with populations of agents that evolve to maximize diversity objectives. However, such approaches are usually greatly less sample efficient than GCRL ones. \svgg approach can be considered as a trade-off between classical GCRL and evolutionary methods, by dealing with a population of goal particles, ensuring diversity and benefiting from sample efficiency of gradient-based optimization. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> save_intro.tex <==

A first approach consists in explicitly modeling the distribution of achieved goals and sampling behavioral goals from a function of this distribution. This is the approach of \skewfit \cite{pong2019skew} or \mega and \omeg \cite{pitis2020maximum}. For instance, by focusing on the border of the distribution of achieved goals, \mega obtains strong exploration results. But doing so, it does not sample again previously achieved goals, preventing performance improvement on these goals. Most importantly, as we will show, always targeting new goals makes it forget about the previous goals, finally resulting in poor success coverage.

A second approach is to implicitly model the current achieved goal distribution through a discriminator which is used to generate goals of intermediate difficulty (GOIDs). This is the approach of \ggan \cite{florensa2017reverse}, asymetric self-play \cite{sukhbaatar2017intrinsic}, \setso \cite{racaniere2019automated} or \vds \cite{zhang2020}. Those methods target more explicitly performance, but generating goals from an adversarial distribution is more unstable.

%Other related unsupervised skill discovery approaches such as \vic \citep{gregor2016variational}, \diayn \citep{eysenbach2018diversity}, \valor \citep{achiam2018variational} or \vgcrl \citep{choi2021variational} look for diversity, but the policy they learn is not conditioned on a goal to be achieved.
